Sample Splitting and Weak Assumption Inference For Time Series

We consider the problem of inference after model selection under weak assumptions in the time series setting. Even when the data are not independent, we show that sample splitting remains asymptotically valid as long as the process satisfies appropriate weak dependence conditions and the functional of interest is suitably well-behaved. In addition, if the inference targets are appropriately defined, we demonstrate that valid statistical inference is possible without assuming stationarity. As a working example, we consider post-selection inference for regression coefficients under a random design assumption, in which the pair $(Y_i, X_i) \in \mathbb{R}^{p_n}$ is assumed to be an observation from a weakly dependent triangular array. We establish (asymptotic) sample splitting validity for regression coefficients under both $\beta$-mixing and $\tau$-dependence assumptions. To facilitate statistical inference in the non-stationary, weakly dependent regime, we extend a central limit theorem of Doukhan and Wintenberger (2007). To extend their result, we derive some properties of the variance of a normalized sum of a weakly dependent process. In particular, we show that, under very general conditions, the variance is often well-approximated by independent blocks. Using this result, we derive the validity of the block multiplier bootstrap under $\theta$-dependence and demonstrate the validity of an inference procedure that combines sample splitting with the bootstrap under weak assumptions.

==> regression_inf.tex <==
We now put together results from the previous sections to derive conditions under which confidence intervals produced by the block multiplier bootstrap after sample splitting provide valid inference for the regression coefficient under a $\tau$-dependence condition.  For simplicity, suppose that a particular coefficient $\beta_{1,\hat{m},n} \in \mathbb{R}$ is of interest; this can easily be generalized to a confidence band or Bonferroni interval.  
In what follows, let $C_{\hat{m},n}^*$ correspond to the confidence set:
\begin{align}
C_{\hat{m},n}^* &= \left[ \hat{\beta}_{1,\hat{m},n} - z_{(1-\alpha)/2}\frac{\sigma_{\hat{m},n}^*}{\sqrt{n}}, \ \hat{\beta}_{1,\hat{m},n} + z_{(1-\alpha)/2}\frac{\sigma_{\hat{m},n}^*}{\sqrt{n}}   \right]
\end{align} 
where $z_{(1-\alpha)/2}$ is the $(1-\alpha)/2$-quantile of the Standard Normal and  $\sigma_{\hat{m}}^*$ is the standard deviation corresponding the bootstrapped regression coefficients.  In the regression coefficient case, the bootstrap distribution is approximated as follows.  Consider a large number $B$ of Monte Carlo iterations.  On the $j$th iteration of the bootstrap, generate $e_1, \ldots, e_{m+1} \sim N(0,1)$ and form the bootstrapped functional $\psi_{n, \hat{m}, j}^{*} = \psi_{n}^{(\hat{m})} + n^{-1/2} W_{n,j}^{(\hat{m})}$.  We may then construct a corresponding bootstrap realization by letting $\hat{\beta}_{1,\hat{m},n,j}^{*} = g^{(m)}(\psi_{n, \hat{m},j}^*)$.  The standard deviation $\sigma_{\hat{m}}^*$ may then be approximated by:
\begin{align}
\sigma_{\hat{m}}^* \approx \sqrt{\frac{1}{B} \sum_{j=1}^B \left(\hat{\beta}_{1,\hat{m},n,j}^* -  \frac{1}{B} \sum_{j=1}^B \hat{\beta}_{1,\hat{m},n,j}^*\right)^2}
\end{align} 
We are now ready to state the following theorem, which establishes validity of sample splitting together with the bootstrap.  The proof relies heavily on several results that we have established in previous theorems.    

\begin{theorem}[Valid Bootstrap Inference for Regression Coefficient after Sample Splitting]  Suppose $\{Y_{n,i}\}$ is a triangular array of random variables such that for each $n,$ $Y_{n,i}$ is a random variable in $\mathbb{R}^{p_n}$ and that the vector has constant mean. Consider a model selection procedure $\hat{m}$ that has the property $P(\hat{m} \in \mathcal{M}^*) \rightarrow 1$ for some $\mathcal{M}^*$ satisfying $|\mathcal{M}^*| < \infty$. For each $m \in \mathcal{M}^*$, suppose that $g^{(m)}(\cdot)$ is differentiable in a neighborhood of $\mathbb{E}[\psi_{n}^{(m)}]$.  Further, for each $m \in \mathcal{M}^*$, suppose that $\theta_r(Y_1^{2n}) = O(r^{-\theta})$ for some $\theta > 4$  the coordinates of $(Y_i^{(m)}, X_{i}^{(m)})$ are $\mathrm{subE}(K_1)$ random variables.
% \end{enumerate} 
% \begin{enumerate}[label=B] 
% \item $\beta_r(Y_1^n)) = O(r^{-(3 + \delta)})$ for some $\delta > 0$ and the coordinates of $(Y_i^{(m)}, X_{i}^{(m)})$ are $\mathrm{subE}(K_1)$ random variables  
% \end{enumerate}
Then,
\begin{align}
P\left( \beta_{1,\hat{m},n} \in C_{\hat{m},n}^* \right) = 1 - \alpha - o(1)
\end{align} 
\end{theorem}


\begin{proof}
By Theorem 


It suffices to show:
\begin{align}
 \mathcal{L}(\sqrt{n}(\hat{\beta}_{1,\hat{m},n} - \beta_{1,\hat{m},n}))  {\overset{wa} \iff} \mathcal{L}(\sqrt{n}(\hat{\beta}_{1,\hat{m},n}^* - \hat{\beta}_{1,\hat{m},n}))
\end{align} 



 \begin{align}
\begin{split}
& \ \ \ P \left( d_{BL} \left[ \mathcal{L}\bigl(\sqrt{n}(\hat{\beta}_{1,\hat{m},n}^* - \hat{\beta}_{1,\hat{m},n}), \widetilde{\mathcal{L}}\bigl(\sqrt{n}(\hat{\beta}_{1,\hat{m},n} - \beta_{1,\hat{m},n}) \bigr) \right] > \epsilon \right)
\\ & \leq \sum_{m \in \mathcal{M}^*}  P \left( d_{BL} \left[ \mathcal{L} \bigl(\sqrt{n}(\hat{\beta}_{1,m,n}^* - \hat{\beta}_{1,m,n}  \bigr), \mathcal{L}\bigl(\sqrt{n}(\hat{\beta}_{1,m,n} - \beta_{1,m,n})\bigr) \right] > \epsilon \right) 
\\ & \ \ \ \ \ \ + P(m \not\in \mathcal{M}^*)
% \\ & \leq \sum_{m^* \in \mathcal{M}^*} P \left\{ d_{BL} \left[ \mathcal{L}(\hat{\theta}_{m^*}(Y_{n+1}^{2n})\ | \ Y_1^n), \mathcal{L}(\hat{\theta}_{m^*}(\widetilde{Y}_{n+1}^{2n}) \right] > \epsilon \right\} + P(\hat{m}^* \not\in \mathcal{M}^* )
\end{split}
 \end{align}
 Therefore it suffices to establish validity for each fixed $m \in \mathcal{M}^*$.  Now observe that:
\begin{align}
\begin{split}
  \mathcal{L}\bigl(\sqrt{n}(\hat{\beta}_{1,m,n}^* - \hat{\beta}_{1,m,n}) \ | \ Y_1^{2n} \bigr) & {\overset{wa(P)} \iff} N(0,\nabla g(\psi_n^{(m)})^T \Sigma_n) 
  \\ &{\overset{wa(P)} \iff} N(0,\nabla g(\mathbb{E}[\psi_n^{(m)}])^T \Sigma_n)
 \end{split}
\end{align}
where the first line follows due Theorem \ref{bootstrap-validity-tau-dependence}, Proposition \ref{theta-preservation}, the Conditional Delta Method (Theorem \ref{delta-method}), and the second line follows from the Continuous Mapping Theorem (Proposition \ref{continuous-mapping}), Lemma \ref{gaussian-characteristic-difference-multivariate}, and the fact that $\psi_n^{(m)} -\mathbb{E}[\psi_n^{(m)}] \xrightarrow{P} 0$.  Now, by Proposition \ref{weakly-approaching-hoeffding}, this implies that:
\begin{align}
\mathcal{L}\bigl(\sqrt{n}(\hat{\beta}_{1,m,n}^* - \hat{\beta}_{1,m,n})\bigr) {\overset{wa} \iff} N(0,\nabla g(\mathbb{E}[\psi_n^{(m)}])^T \Sigma_n)
\end{align}

 Now, by the Conditional Delta Method and the Central Limit Theorem (Theorem \ref{multivariate-clt}), we also have that:
%
\begin{align}
 \mathcal{L}\bigl(\sqrt{n}(\hat{\beta}_{1,m,n} - \beta_{1,m,n}) \bigr) {\overset{wa} \iff}  N(0,\nabla g(\mathbb{E}[\psi_n^{(m)}])^T \Sigma_n) 
\end{align}

The result follows.  
% \begin{align}
% \begin{split}
% \mathcal{L}(\hat{\theta}_{m^*}(Y_{n+1}^{2n})) & \overset{wa}{\underset{(1)} \iff }  \mathcal{L}(\hat{\theta}_{m^*}(Y_{n+i_n+1}^{2n})) \overset{wa(P)} {\underset{(2)} \iff} \mathcal{L}(\hat{\theta}_{m^*}(Y_{n+i_n+1}^{2n}) |Y_1^n) 
% \\ & \overset{wa(P)} {\underset{(3)} \iff} \mathcal{L}(\hat{\theta}_{m^*}(Y_{n+1}^{2n}) |Y_1^n)
% % \overset{wa(P)} {\underset{(4)} \iff} \mathcal{L}(\hat{\theta}_{\hat{m}}(Y_{n+1}^{2n}) |Y_1^n)
% \end{split}
% \end{align}

\end{proof}

